Huawei Cloud Model-as-a-Service on the CloudMatrix384 SuperPod

Scaled-out MoE LLMs and scaled-up SuperPods create new systems challenges for production Model-as-a-Service (MaaS), requiring disaggregation, low-latency communication, and decentralized serving. This report presents xDeepServe, the production serving system behind Huawei Cloud's MaaS offering on CloudMatrix384, a 48-server SuperPod with 384 Ascend 910C chips connected by a high-bandwidth UB fabric and global shared memory. It serves models including DeepSeek, Kimi, GLM, Qwen, and MiniMax, among others. xDeepServe is built around Transformerless, a disaggregated execution architecture that decomposes transformer inference into modular units -- attention, feedforward, and MoE -- and supports disaggregated Prefill-Decode and MoE-Attention deployments. To enable disaggregation, we develop XCCL, a memory-semantic communication layer providing microsecond-level point-to-point and scalable all-to-all primitives, and we extend FlowServe with decentralized DP groups and techniques to mitigate stragglers and synchronization variance. In a peak decoding configuration, xDeepServe reaches 2400 tokens/s per Ascend 910C chip at ~50ms time-per-output-token (TPOT).

==> Content/background.backup.tex <==
\subsection{NPU Execution Mode}

\input{Figures/fig-graph-mode}

Frameworks such as PyTorch represent neural networks as computation graphs (Figure~\ref{fig-graph-mode} (a)). To execute these graphs, they typically support two execution modes: eager mode and graph mode.


\textbf{Eager Mode.}
%
Eager mode is the default execution mode in PyTorch. In this mode, each operator is dispatched to the NPU immediately upon invocation in Python, returning results that can be directly inspected, modified, or reused. This imperative and dynamic behavior supports arbitrary control flow (e.g., loops and conditionals), Python-native debugging tools, and dynamic tensor shapes. Consequently, eager mode offers an intuitive and interactive programming experience, particularly suited for development, debugging, and experimentation.

However, this flexibility comes at the cost of performance. First, the host must launch each operator individually, introducing significant host-side overhead. As shown in Figure~\ref{fig-graph-mode}(b), when operator execution is compute-intensive (e.g., during the prefill stage), the host-side overhead is negligible. In contrast, when operator execution is lightweight (e.g., during the decode stage), the host-side overhead dominates, resulting in underutilized NPUs (Figure~\ref{fig-graph-mode}(c)). Second, the immediate execution of each operation prevents whole-graph analysis and optimizations such as operator fusion. For instance, although Matrix Multiplication (MM) and ReLU are well-suited for fusion, eager mode executes them sequentially, prohibiting such optimization (Figure~\ref{fig-graph-mode}(a)(b)(c)).

\textbf{Graph Mode.}
%
To improve performance in production scenarios, frameworks such as PyTorch provide an optional graph mode. In this mode, operators are not executed immediately; instead, they contribute to constructing a static, declarative computation graph, which can be globally analyzed, optimized, and dispatched to the NPU as a whole. PyTorch supports graph mode primarily for GPUs through tools such as TorchDynamo and TorchCompile, which trace and optimize Python code into an intermediate representation. In contrast, Huawei targets NPUs using tools such as PTA (PyTorch Adapter) and TorchAIR, which perform similar tracing and static compilation to leverage NPU-specific acceleration.


As a result, the graph mode offers the following performance advantages. First, the framework can dispatch the entire computation graph to the NPU like a single operator, eliminating per-operator launch overhead. As shown in Figure~\ref{fig-graph-mode}, the NPU can execute the whole graph without waiting for host intervention, improving hardware utilization. Second, the static graph enables global compiler optimizations, such as operator fusion, dead code elimination, and constant folding. As shown in Figure~\ref{fig-graph-mode}, operator fusion alone further reduces the latency and memory usage with in-place computation.

\textbf{Execution Modes for Prefill and Decode Stages.}
%
As discussed in detail in Section~\ref{}, we adopt different execution modes for the prefill and decode stages.

The prefill stage employs eager mode for two reasons. First, its input shapes are dynamic. Specifically, the batch size varies depending on the number of incoming requests, making it difficult to construct a static computation graph. Second, eager execution does not hinder performance in the prefill stage. Prefill involves computationally intensive operations such as processing long sequences and performing dense matrix multiplications, making it device-bound. Thus, the overhead of eager execution is effectively hidden by the heavy kernel workload.

In contrast, the decode stage employs graph mode for two reasons. First, input shapes in decode are static, as the number of tokens packed into each batch is predetermined. This allows for the construction of a static computation graph. Second, decode is compute-light and memory-bound; if executed in eager mode, frequent host launches dominate runtime, resulting in underutilized NPUs. Graph mode eliminates this overhead by enabling the NPU to execute the entire graph without host intervention, improving overall efficiency.

==> Content/tmp-google-colab.tex <==

import matplotlib.pyplot as plt
import numpy as np

# Data extracted from the pie chart
labels = [
    'QuantBatchMatmul', 'MoE-Combine', 'MoE-Dispatch',
    'MultiLatentAttention', 'MlaPreprocess', 'Others'
]

sizes = [
    22.08, 20.39, 15.31,
    21.85, 8.69,  11.69
] 

# ColorBrewer Set2 palette: clean, readable, paper-friendly
colors = ['#66c2a5', '#fc8d62', '#8da0cb',
          '#e78ac3', '#a6d854', '#ffd92f']

# Sort the data by descending size
sorted_data = sorted(zip(sizes, labels, colors), reverse=True)
sizes, labels, colors = zip(*sorted_data)

# Plot
fig, ax = plt.subplots(figsize=(8, 8))
fig.patch.set_facecolor('white')
ax.set_facecolor('white')

# Draw pie chart with only percentages inside
wedges, texts, autotexts = ax.pie(
    sizes,
    labels=None,
    autopct='%1.1f%%',
    startangle=90,
    colors=colors,
    textprops={'color': 'black', 'fontsize': 18, 'weight': 'bold'}
)

# Add labels slightly outside the pie to avoid overlap
for i, wedge in enumerate(wedges):
    angle = (wedge.theta2 + wedge.theta1) / 2.0
    angle_rad = np.deg2rad(angle)
    x = 1.1 * np.cos(angle_rad)
    y = 1.1 * np.sin(angle_rad)
    ax.text(x, y, labels[i], ha='center', va='center', fontsize=18, color='black')

ax.axis('equal')
plt.style.use('seaborn-v0_8-pastel')

# Save without extra white space
plt.savefig('fig-2400-operator-pie.pdf', format='pdf', bbox_inches='tight', pad_inches=0)
plt.show()













import matplotlib.pyplot as plt
import numpy as np

# 数据准备
kb_sizes = ['MoE-Dispatch', 'MoE-Combine']
threads = [4, 8, 16, 32, 64, 80, 96, 128]  # 更方便地与 data 对齐

data = [
    [40.8, 42.4, 46.1, 54.3, 79, 92.8, 101.3, 123.5],
    [27.6, 31.7, 41.3, 57.7, 84.6, 105.5, 110.4, 143.4],
]

# 检查 data 长度是否与 threads 对应
min_len = min(len(threads), len(data[0]))
threads = threads[:min_len]  # 确保与 data 对齐

# 使用前两个颜色
dark_colors = [
    '#1f77b4',  # Dark Blue
    '#ff7f0e',  # Burnt Orange (slightly darkened)
]

plt.figure(figsize=(8, 7))
plt.style.use('seaborn-v0_8-pastel')  # 使用美观样式

# 为每种KB大小绘制折线
for i in range(len(kb_sizes)):
    y_values = data[i][:min_len]  # 确保 y 长度正确
    plt.plot(
        threads,
        y_values,
        marker='o',
        label=kb_sizes[i],
        linewidth=2.5,
        markersize=8,
        color=dark_colors[i]
    )

# 添加图例和标签
plt.xlabel('Batch Size per Die (EP128)', fontsize=22)
plt.ylabel('Latency (us)', fontsize=22)
plt.legend(loc='lower right', fontsize=18)

# 调整坐标轴和网格
plt.grid(True, linestyle='--')
plt.xticks(threads, fontsize=16)
plt.yticks(fontsize=16)
plt.ylim(0, max([max(row[:min_len]) for row in data]) * 1.1)

# 调整布局防止标签重叠
plt.tight_layout()

# 保存图像
plt.savefig('fig-xccl-dispatch-combine.pdf', format='pdf', bbox_inches='tight')
plt.show()























import matplotlib.pyplot as plt
import numpy as np

# 数据准备
kb_sizes = ['MoE-Native', 'MoE-Balanced', 'MoE-Avg-Routing']
threads = [8, 16, 32, 64, 80, 96, 144, 192]  # 更方便地与 data 对齐

data = [
    [30.48, 35.89, 46.36, 70.21, 82.01, 91.71, 122.44, 150.24],
    [29.00, 31.3, 38.38, 53.64, 59.4, 66.51, 87.64, 106.82],
    [28.87, 30.99, 37.26, 51.09, 56.03, 62.45, 81.53, 98.91],
]

# 检查 data 长度是否与 threads 对应
min_len = min(len(threads), len(data[0]))
threads = threads[:min_len]  # 确保与 data 对齐

# 使用前两个颜色
dark_colors = [
    '#1f77b4',  # Dark Blue
    '#ff7f0e',  # Burnt Orange (slightly darkened)
    '#2ca02c',  # Dark Green
]

plt.figure(figsize=(8, 7))
plt.style.use('seaborn-v0_8-pastel')  # 使用美观样式

# 为每种KB大小绘制折线
for i in range(len(kb_sizes)):
    y_values = data[i][:min_len]  # 确保 y 长度正确
    plt.plot(
        threads,
        y_values,
        marker='o',
        label=kb_sizes[i],
        linewidth=2.5,
        markersize=8,
        color=dark_colors[i]
    )

# 添加图例和标签
plt.xlabel('Batch Size per Die', fontsize=22)
plt.ylabel('Latency (us)', fontsize=22)
plt.legend(loc='lower right', fontsize=18)

# 调整坐标轴和网格
plt.grid(True, linestyle='--')
plt.xticks(threads, fontsize=16)
plt.yticks(fontsize=16)
plt.ylim(0, max([max(row[:min_len]) for row in data]) * 1.1)

# 调整布局防止标签重叠
plt.tight_layout()

# 保存图像
plt.savefig('fig-moe-lb-motivation-perf.pdf', format='pdf', bbox_inches='tight')
plt.show()

==> Figures/fig-dynamic-mb.tex <==
\begin{figure}[th]
    \centering
    \includegraphics[width=\textwidth]{Figures/figs/fig-dynamic-mb.png}
    \caption{Dynamic MicroBatch}
    \label{fig-dynamic-mb}
\end{figure}

==> Figures/fig-eval-accuracy.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{Figures/figs/fig-eval-accuracy.pdf}
    \caption{Accuracy Benchmark. \ys{pls replace this with pyplot geneated PDF figures.}}
    \label{fig-eval-accuracy}
\end{figure}

==> Figures/fig-eval-moe-lb.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/figs/xxx.pdf}
    \caption{MoE-LB Study. \ys{We need (1) MoE-Heatmap before and after LB; (2) TTFT/TPOT change after MoE-LB; (3) we can compare dynamic-MoE-LB, or dynamic-balanced-XCCL-dispatch.}}
    \label{fig-eval-moe-lb}
\end{figure}

==> Figures/fig-eval-network.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{Figures/figs/fig-eval-network.pdf}
    \caption{Low-level Hardware and XCCL Performance.}
    \label{fig-eval-xccl}
\end{figure}

==> Figures/fig-jitter.tex <==
\begin{figure}[th]
    \centering
    \includegraphics[width=\textwidth]{Figures/figs/fig-jitter.png}
    \caption{Graph launch jitter illustration. \ys{replot this figure.}}
    \label{fig-jitter}
\end{figure}

==> Figures/fig-prefix-caching.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{Figures/figs/fig-prefix-caching.png}
    \caption{Prefix Caching E2E Design. \ys{show prefix matching, saving workflow, replace ems with rtc c++ threads.}}
    \label{fig-prefix-caching}
\end{figure}

==> Figures/fig-system-overview.tex <==
%
% You can find the drawing below:
% https://docs.google.com/drawings/d/11Elh-iu1a1mXVCSdSYV58hv83c9RVQRnn-Q4wfA5dms/edit?usp=sharing
%

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{Figures/figs/fig-system-overview.pdf}
    \caption{\textbf{\xds Architecture over \cloudmatrix.}}
    \label{fig-system-overview}
\end{figure}

==> Figures/fig-xccl-a2e-eval.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/figs/xx.pdf}
    \caption{\textbf{Evaluation of A2E/E2A.} \textit{XXXX}}
    \label{fig-xccl-a2e-e2a-eval}
\end{figure}

==> Figures/fig-xccl-dispatch-combine-eval.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/figs/XX.pdf}
    \caption{Eval of Dispatch.}
    \label{fig-xccl-dispatch-eval}
\end{figure}

==> Figures/fig-xccl.tex <==
%
% https://docs.google.com/drawings/d/1eD96rU4WWLt7tRz87MRFTnAbiF9fWtBeTUZhdr0Wvgw/edit
%


\begin{figure}[h]
    \centering
    \includegraphics[width=0.65\textwidth]{Figures/figs/fig-xccl-overview.pdf}
    \caption{An Overview of \xccl.}
    \label{fig-xccl-overview}
\end{figure}

==> README.tex <==
\section{Rules} 

\subsection{What TODO}
\begin{itemize}

\item Always follow the organization and naming styles of existing files/folders. For example, put figures, tables, and content into the corresponding folders.

\item Add the figures into the figures/figs folder and their corresponding texts into the figures/ folder. The reason for doing this is to avoid Arxiv's naming conflicts within the same folder level.

\item Always use .pdf figures. Never use other formats such as .png, .jpeg, and so on.

\item Add necessary packages in package.tex, and add necessary new commands in macro.tex.


\end{itemize}

\subsection{What NOT TODO}
\begin{itemize}

\item Never change the content of the xds.cls file. If the change is necessary, please get in touch with the project owner.

\item Never change the names of the first-level files such as main.tex, main.bib, xds.cls, and so on.


\end{itemize}
